Spacetime metric for pedestrian movement

This paper will present a model for pedestrian motion by defining a spacetime metric. This model considers the factors that are effective in the movement of pedestrians (such as obstacles, walls and other pedestrians) by defining a proper metric. In fact, the surrounding environment that affects the motion of pedestrians changes the flat(Euclidean) spacetime metric and, therefore, the shortest possible path to their destination. This change is such that pedestrians have a different feeling of time at any point and moment in the environment. Based on this feeling, they adjust their route to the destination so that they travel the shortest possible route in curved spacetime, which follows a geodesic. The contributions are :1. Defining spacetime metric for pedestrian movement.2. Visualizing the spacetime geometry for several timesteps.3. Introducing a parameter called the time factor and its physical meaning in terms of the pedestrian feeling of time. According to this paper formulation, pedestrians feel time differently at each position and moment, and the time factor measures this feeling of time. 4. Proposing a simple model with differential equations suitable for data assimilation methods while preserving the essential feature of collision avoidance behaviour.

==> sections/equation.tex <==
\section{Equation of motion in classical mechanics}\label{classic}
\noindent From classical mechanics, we know that:

\begin{align}
\overrightarrow{F}=-m\overrightarrow{\nabla }U\\
\overrightarrow{a}=-\overrightarrow{\nabla }U=-\frac{\partial U}{\partial r}\overrightarrow{e}_{r}-\frac{1}{r}\frac{\partial U}{\partial \theta}\overrightarrow{e}_{\theta }
\end{align}

\noindent Also, by differentiating $\overrightarrow{{r}}{=r}{\overrightarrow{{e}}}_{{r}}$ we get:

\begin{equation}
 {\overrightarrow{{a}}}=(\ddot{{r}}{-}{r}{\dot{{\thetaup }}}^{{2}}{)}{\overrightarrow{{e}}}_{{r}}{+(r}\ddot{{\thetaup }}{+2}\dot{{r}}\dot{{\thetaup }}{)}{\overrightarrow{{e}}}_{\theta } 
\end{equation}

Therefore:

\begin{align}
-\frac{\partial U }{\partial r }=\ddot{r}-{r}\dot{\thetaup }^{2}\\
-\frac{1}{r}\frac{\partial U}{\partial \theta}={r}\ddot{\thetaup }+2\dot{r}\dot{\theta}
\end{align}


Which are the same equations as Eq. (\ref {modern1},\ref {modern2}). By proving that the geodesic equation is the same as the classical mechanics' equation (Sec.[\ref{modern},\ref{classic}]), we conclude that the proposed metric describes the motion in the same way as classical mechanics. 




==> sections/utility.tex <==
\section{Utility function for metric construction}\label{utility}
** This section is in progress **


There are strong similarities between utility function and potential function. First, for both utility and potential function, the level is immaterial. Second, both functions provide a measure of distance. This was the primary reason I opted to incorporate potential functions for defining the metric in previous sections. As for the utility function, the measure of distance property is more tangible in the route choice problem \cite{fosgerau2013link,NASSIR2019528} as the main problem being solved is the shortest path problem considering the physical limitations of the route choice problem\cite{ZIMMERMANN2020100004}. We will discuss how this approach will increase the accuracy and sophistication of pedestrian modelling. Using utilities paves the way to digest real-world experiments data into the metric method. In this section, we plan to define the metric based on the utility function. We do this based on virtual reality experiments.


